A Distributed Second-Order Algorithm You Can Trust

Due to the rapid growth of data and computational resources, distributed optimization has become an active research area in recent years. While first-order methods seem to dominate the field, second-order methods are nevertheless attractive as they potentially require fewer communication rounds to converge. However, there are significant drawbacks that impede their wide adoption, such as the computation and the communication of a large Hessian matrix. In this paper we present a new algorithm for distributed training of generalized linear models that only requires the computation of diagonal blocks of the Hessian matrix on the individual workers. To deal with this approximate information we propose an adaptive approach that - akin to trust-region methods - dynamically adapts the auxiliary model to compensate for modeling errors. We provide theoretical rates of convergence for a wide class of problems including L1-regularized objectives. We also demonstrate that our approach achieves state-of-the-art results on multiple large benchmark datasets.

==> 02_method_cdu.tex <==
% !TEX root = icml-hessian-cocoa.tex

\section{Method Description}
\label{sec:method}

We present an iterative descent algorithm that minimizes the objective introduced in Eq.~\eqref{eq:A}. At each step, we optimize an auxiliary \emph{block-separable model} that acts as surrogate for the objective in Eq.~\eqref{eq:A}. We first introduce the block-separable model motivated by trust region and then present our algorithm used to optimize Eq.~\eqref{eq:A}.

\subsection{Block-Separable Model}
\label{sec:block_model}
The objective \eqref{eq:A} consists of two terms. Where the first term makes the optimization task challenging in a distributed setting since it does not separate over partitions. Let us consider the following auxilary model for $f$ at every iteration:
\begin{align} f(A(\alphav+\Dav)) \approx & f(A\alphav) \notag\\&+ \nabla f(A\alphav)^\top A\Dav
\label{eq:modelCoCoA}\\&+\frac 1 {2}(A\Dav)^\top M  A\Dav.\notag
\end{align}
with 
\[M:=\sigma_1 \nabla^2 f(A\alphav) +\sigma_2 I\]
For $\sigma_1=1$ and $\sigma_2 =0$ thsi corresponds to a classical second order approximation, if $\sigma_2$ is non-zero it corresponds to a classical trust regin approach for optimizing $f$, where $\sigma_2$ corresponds to the trust region radius. \\
However, optimizing \eqref{eq:modelCoCoA} requires  access to the full correlation matrix which is not feasible in a distributed setting where the data is partitioned among the workers. In particular, we assume each worker has access to a subset $\cI_k$ of the columns of $A$. In our setting, $\cI_k$ are disjoint index sets such that
\[ \bigcup_k \cI_k = [n], \;\;\cI_i \cap \cI_j = \emptyset \;\; \forall i\neq j\] 
and $n_k := \left|\cI_k\right|$ denotes the size of partition $k$. Hence, each machine stores in its memory the submatrix $A_{[k]}\in\R^{d \times n_k}$ corresponding to its partition $\cI_k$.

Therefore, given such a partitioning we suggest that in each step, every worker works on its own the following local approximation of $f$  based on its own local partition of the data, i.e. 
\begin{align} \tilde f^{(k)}(\alphav, \Dak)&:=  f(\vv) \notag\\&+ \nabla f(\vv)^\top A_{[k]}\Dav\notag\\&+\frac 1 {2}(A_{[k]}\Dav)^\top M  A_{[k]}\Dav.
\notag
\end{align}
where we assume the informaiton $\vv:=A\alphav$ about the previous stage of the algorithm is shared among all workers.

Hence, considering all the workers, in every iteration of a distributed algorithm, the following surrogate would be optimized which separates over the $K$ partitions as
\[\model_{\sigma}(\Dav; \alphav) = \sum_k \msk(\Dak; \alphav),\] 
with
\begin{align}  \msk(\Dak; \alphav)  &:= \frac 1 K f(\vv) +\nabla f(\vv)^\top A\Dak\notag \\&+ \frac {1} 2 \sum_k (A_{[k]}\Dav)^\top M (A_{[k]}\Dav) .\notag\\
&+\sum_{i\in\cI_k} g_i((\alphav+\Dak)_i) 
\label{eq:localModel}
\end{align}
where every subproblem $\msk(\Dak; \alphav)$ only requires access to a single partition of the data. We use the notation $\uv_{[k]}$ to denote the vector $\uv$ with only non-zero coordinates for $i\in \cI_k$.

A significant benefit of this model is that it is based on local second order information and does not require sending gradients and Hessian matrices to the master node, which would be a significant cost in terms of communication.

\subsection{Approximation Quality of the Model}
%The approximation quality of the model is measured by the $\sigma$ parameter as this parameter accounts for the loss of information that arises by enforcing the approximate Hessian matrix of $f$ to have a block diagonal structure.
%This parameter has a central role for the convergence and the practical performance of our method, and we therefore need an efficient way to update this parameter. The update rule that will be detailed in the next section acts as the reciprocal of the trust-region radius used by trust-region methods~\cite{Cartis2011}.
% al: we can change this description if you think it's still misleading

The role of the $\sigma$ parameter is to account for the loss of information that arises by enforcing the approximate Hessian matrix of $f$ to have a block diagonal structure. The better the approximation is, the closer to $1$ the $\sigma$ parameter can be chosen. This parameter has a central role for the convergence and the practical performance of our method, and we therefore need an efficient way to choose and update this parameter. 
 The update rule that will be detailed in the next section is inspired by  trust-region methods~\cite{Cartis2011}, where $\sigma$
 %is it (1-\sigma)? 
 acts as the reciprocal of the trust-region radius.


%the trust region approach adjusts its value in an online fashion based on the results of the previous iteration. In this perspective, $\sigma$ can be interpreted as the radius defining the region where our local model constitutes a valid approximation of the original function.  %cdu: I am not sure radius is the best way to think of \sigma...
%discuss role of $\sigma$.

% Don't need this definition here, could move it to the appendix later.
%\paragraph{$\sigma$ Definition}
%\begin{equation}
%\sigma \geq \sigma_{min} := \max_{\substack{\alphav, \Dav, \\ \theta \in [0,1]}} \frac{\Dav^\top \nabla f^2(A(\alphav + \theta\Dav))  \Dav}{\Dav^\top \tilde{H}(\alphav)  \Dav} 
%\end{equation}

\subsection{Algorithm Procedure}
The pseudo-code of the proposed algorithm is given in Algorithm~\ref{alg:adaptive_cocoa}. At every round, every worker $k$ works on its local subproblem \eqref{eq:localModel}, to find an update $\Dak$. Then every worker communicates its update to the master which aggregates them and updates the model as 
\[\alphav^{(t+1)}:=\alphav^{(t)}+\sum_k \Dak.\]
The cost of communication required for Algorithm~\ref{alg:adaptive_cocoa} is minimal as no gradient or Hessian information has to be communicated between the workers and the master node.

The local subproblems \eqref{eq:localModel} do not necessarily need to be solved exactly but can be solved $\eta$-approximately, i.e., the local updates $\Dak$ are such that:
\begin{align}
\frac{\msk(\Dak; \alphav)- \msk(\Dav^\star_{[k]}; \alphav)}{\msk(\0; \alphav)-\msk(\Dav^\star_{[k]}; \alphav)}\leq \eta\, ,
\label{eq:theta_approx}
\end{align}
where $\Dav^\star_{[k]} = \argmin_\Dak \msk(\Dak; \alphav)$.

As previously mentioned, one of the key step in the adaptive approach presented in Algorithm~\ref{alg:adaptive_cocoa} is the strategy for adapting the model as the algorithm proceeds. This is done by choosing $\sigma$ appropriately in every iteration $t$ resulting in schedule for $\sigma$ described by the sequence $\{\sigma_t\}_{t\geq0}$. 
%al: do you have a better idea how to introduce \sigma_t?
In every iteration, we base the choice of $\sigma$ on the agreement between the model function \eqref{eq:modelCoCoA} and the objective function \eqref{eq:A}, which is represented by the variable $\rho_t$ defined in Eq.~\eqref{eq:rho} in Algorithm~\ref{alg:adaptive_cocoa}. If $\rho_t$ is negative, the new objective value is greater than the current value, so the step is rejected. 
On the other hand, if $\rho_t$ is close to $1$ there is a good agreement between the model $m_{\sigma_t}$ and the function $\bO$ over this step and we can trust our model. If our model overestimates the objective we decrease $\sigma$ for the next iteration, which can be thought of as putting more trust in the current approximation of the Hessian. If our model underestimates the objective we increase $\sigma$.
%al: I updated the discussion for $\sigma$, i.e. it's the reciprocal of the TR radius, same as Cartis11.
%cdu: I guess I was confused because sigms = 1 is optimal not \sigma = 0. But I think the TR xorresponds to 1/(1-sigma) - right?

 \begin{algorithm}[h!]
   \caption{Adaptive Scheme ({\color{red} name?})}
   \label{alg:adaptive_cocoa}
\begin{algorithmic}[1] 
   \STATE {\bfseries Input:} \\ 
   %$\quad$ training examples $\S = (\x_1,\x_2,\ldots,\x_n)$, $\x_i \sim P$\\
   $\quad$ Starting point $\alphav_0 \in \R^n$ (e.g~$\alphav_0 = {\bf 0}$) \\
   $\quad$ $\sigma_0>0$\\
   $\quad  \gamma_2>1>\gamma_1>0$, $\zeta_2\geq1\geq\zeta_1>0$, and $\xi>0$
   \FOR{$t=0,1,\dots,\text{until convergence}$}
     \FOR{$k\in[K] \text{ in parallel}$}
   \STATE Obtain $\Dak$ by minimizing $\mstk(\Dak; \alphat)$ $\eta$-approximately
	\ENDFOR
	\STATE Aggregate updates $\Dav = \sum_k\Dak$  
   \STATE Compute $\bO(\alphav^{(t)}+ \Dav)$ and 
	\begin{equation}
	\rho_t=\dfrac{\bO(\alphav^{(t)})-\bO(\alphav^{(t)}+ \Dav)}{\bO(\alphav^{(t)})-m_{\sigma_t}(\Dav; \alphat)}
	\label{eq:rho}
	\end{equation}
	\STATE Set
	\begin{equation}
	\alphav^{(t+1)} = \begin{cases}
	\alphav^{(t)} + \Dav & \text{ if } \rho_t \geq \xi \\
	\alphav^{(t)} & \text{ otherwise}
	\end{cases}
	\end{equation}
	\STATE Set
	\begin{equation} \label{eq:sigma_update}
	\sigma_{t+1}= \begin{cases}
	\sigma_t \gamma_1 & \text{ if } \rho_t>\zeta_2 \text{ (too conservative) }\\
	\sigma_t & \text{ if } \zeta_2\geq\rho_t\geq \zeta_1 \text{ (good fit)}\\
	\sigma_t \gamma_2& \text{ if } \zeta_1>\rho_t \text{ (too aggressive)},
	\end{cases}
	\end{equation}
   \ENDFOR
\end{algorithmic}
\end{algorithm}
